AccelGen: Heterogeneous SLO-Guaranteed High-Throughput LLM Inference Serving for Diverse Applications

In this paper, we consider a mixed-prompt scenario for a large language model (LLM) inference serving system that supports diverse applications with both short prompts and long prompts and heterogeneous SLOs for iteration time. To improve throughput when handling long prompts, previous research introduces a chunking method, but has not addressed heterogeneous SLOs. To address the limitation, we propose AccelGen, a high-throughput LLM inference serving system with heterogeneous SLO guarantees for diverse applications. AccelGen introduces four core components: (1) SLO-guaranteed dynamic chunking, which dynamically adjusts chunk sizes to maximize GPU compute utilization while meeting iteration-level SLOs; (2) Iteration-level SLO-based task prioritization, which prioritizes tight-SLO requests and batches requests with similar SLOs; (3) Multi-resource-aware batching, which selects queued requests to maximize the utilizations of both GPU compute resource and key-value cache (KVC). Trace-driven real experiments demonstrate that AccelGen achieves 1.42-11.21X higher throughput, 1.43-13.71X higher goodput, 37-90% higher SLO attainment, and 1.61-12.22X lower response latency compared to the state-of-the-art approaches. It achieves performance near the Oracle, which optimally maximizes goodput.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> background.tex <==
\DEL{\begin{figure}
    \centering
\includegraphics[width=0.9\columnwidth,height=0.145\textheight]{Fig/transformers-2.png}
    \caption{Transformer layer of GPT.}
    \label{fig:transformer}
\end{figure}}

\DELMayNeed{\noindent{\textbf{Transformer Model.}} We first introduce the transformer model architecture as shown in Figure~\ref{fig:transformer}.} %As a representative of the transformer model, we describe the GPT structure. GPT is a decoder only transformer model. Among the operations that compose the
%Transformer layer, Attention is the essence that distinguishes
%Transformer from other architectures.
%As shown in Figure~\ref{fig:transformer}, \DEL{before the attention layer, GPT transformer consists of the layer normalization operation (LayerNorm) and the QKV Linear (linear and split operations to get the query, key, and value). Operations performed after Attention are, in order, a linear operation (Attn Out Linear), an add operation for residual connection (Add), layer normalization operation (LayerNorm), the fully connect layers (FC) operations, and the other residual
%connection operation (Add). These layers can be divided into two categories: 1) forward computation layers (FCL), and 2) attention layer (marked within a dashed box) in Figure~\ref{fig:transformer}. Rest of the layers marked within the solid box are part of the FCL.
%However, among all these layers attention layer plays the most important role.

\DELMayNeed{
\DEL{($\mathbf{E}$) using three learned metrics $\mathbf{W_q},\mathbf{W_k}$ and $\mathbf{W_v}$}}The three input components to the attention layer, Query ($\mathbf{Q}$), Key ($\mathbf{K}$), and Value ($\mathbf{V}$), are the projections of the embeddings of the transformer. \DEL{The embedded matrix for the whole token sequence input is $\mathbf{E}$, where $e_i$ is the embedding of the each token in the sequence. %So, $\mathbf{E}$ consists of all the tokens in the sequence.
Then, the projection of  is created by
\begin{equation*}
    \mathbf{Q} = \mathbf{W_q} \mathbf{E} \text{, }
    \mathbf{K} = \mathbf{W_K} \mathbf{E} \text{, }
    \mathbf{V} = \mathbf{W_v} \mathbf{E}
\end{equation*}
The projection calculation involves matrix multiplications between the learned matrices and the embedded matrix. At the layer level, each matrix multiplication is a fully connected layer with input and output neurons.} Then, for each matrix multiplication, the number of operations at a layer equals:\vspace{-0.1in}
\begin{equation}\label{equ:opeNum1}
2 \times S_f \times H^2, \vspace{-0.05in}
\end{equation}where $S_f$ denotes the foward size and $H$ is the model dimension. Table~\ref{tab:NotationTable} in Appendix lists a summary of the notations used in the paper. The Attention operation %first calculates the dot products $\mathbf{QK}^T$ that measures the similarity of previous tokens from the query token's perspective and then applies the Softmax to the dot products to get weights and
produces the output: \vspace{-0.2in}
}
%(i.e., attention score)

\DEL{($Self$$-$$attention(\mathbf{Q,K,V}$)) as a weighted sum of the values. Here, the weights are called attention score of the query tokens with respect to the previous tokens. %associated with the weights. %The softmax function ensures that the weights for each Value are positive and sum to 1.
}

\DEL{\begin{equation}
\label{eq:4}
    \mathbf{S} = softmax(\mathbf{QK}^T)
\end{equation}
\begin{equation}
\label{eq:5}
Self-attention(\mathbf{Q,K,V}) = [WeightedSum(\mathbf{V_1,S}),\cdots, WeightedSum(\mathbf{V_n,S})]
\end{equation}
All these mathematical operations can be summarized as follows:}

\DELMayNeed{
\vspace{-0.1in}
\begin{equation}
    \label{eq:6}
    Self-attention(\mathbf{Q,K,V}) = softmax(\frac{\mathbf{QK}^T}{\sqrt{d_k}}) \mathbf{V}, \vspace{-0.05in}
\end{equation} where %$\mathbf{Q}$, $\mathbf{K}$, and $\mathbf{V}$ are the Query weighted matrix, Key weighted matrix and Value weighted matrix, respectively.
$d_k$ (??is $d_k$ H?) is the dimension of the $\mathbf{K}$ or $\mathbf{Q}$. The number of operations at the layer level equals: \vspace{-0.1in}
\begin{equation}\label{equ:opeNum2}\vspace{-0.05in}
4 \times S_f^2 \times H. \vspace{-0.1in}
\end{equation}
}

%So, the whole self attention operation primarily involves two sets of matrix multiplication: 1) $\mathbf{QK}^T$ and 2) out put of the first matrix multiplication with $\mathbf{V}$. So, again considering



%??give computation complexity and also the CV cache size - done
%Such one set of computations is performed by an attention head. There can be multiple heads in a model, and these heads are executed in parallel.}
%4 \times model\_dim \times tokens^2$)

%The output of the transformer layer is the probability of each word to be present in the output. %(??query token is input token or vocabulary token).
%The term ``logits refers to the raw outputs of a model before they are transformed into probabilities. Specifically,



%Logits are the unnormalized outputs of the last layer of a transformer layer (i.e., the FC2 layer).

\DEL{\tannsdi{Let us mathematically explain the attention score calculation process in details. Given a sequence of input tokens $\mathbf{x_1,} \cdots \mathbf{x_n}$ where any $x_i \in \mathbb{R}^d$, %(??explain $\mathbb{R}^d$$),
its self-attention outputs a sequence of the same length $y_1,\cdots,y_n$, where function mapping to learn is as follows.
\begin{equation}
\label{eq:1}
 y_i = f(x_i,(x_1,x_1),\cdots, (x_n,x_n)\in \mathbb{R}^d
\end{equation}
Now, as mentioned above, the attention contains three major components, which are Query ($\mathbf{Q}$), Key($\mathbf{K}$), and Value($\mathbf{V}$) matrices, which are derived from three learned matrices $\mathbf{W_Q},\mathbf{W_K},$ and $\mathbf{W_V}$. A projection of the mentioned $\mathbf{Q}$, $\mathbf{K}$ and $\mathbf{V}$ can be created as follows from the embedding of the embedding of each input token $\mathbf{e_i}$.
\begin{equation}
\label{eq:2}
%\begin{multline}
    \mathbf{Q_i}=\mathbf{W_Q}\mathbf{e_i},
\mathbf{K_i}=\mathbf{W_K}\mathbf{e_i},
\mathbf{V_i}=\mathbf{W_V}\mathbf{e_i}
%\end{multline}
\end{equation}
Then the dot-product similarity between the Query ($\mathbf{Q}$) and Key ($\mathbf{K}$) is being calculated.
\begin{equation}
    \label{eq:3}
    Similarity(\mathbf{Q,K}) = \mathbf{QK}^T
\end{equation}
After the computation the similarity between the $\mathbf{Q}$ and $\mathbf{K}$, the softmax function is applied to obtain the weights. The softmax function ensures that the weights for each Value are positive and sum to 1.
\begin{equation}
\label{eq:4}
    \mathbf{S} = softmax(\mathbf{QK}^T)
\end{equation}
Then, the final output matrix (\mathbf{y}) is obtained by concatenating the Weighted Sum matrices computed for each embedding in the input sequence:
\begin{equation}
\label{eq:5}
\mathbf{y} = [WeightedSum(\mathbf{V_1,S}),\cdots, WeightedSum(\mathbf{V_n,S})]
\end{equation}
Finally, the  Self-attention score calculation mechanism can be summarized with the following formula:
\begin{equation}
    \label{eq:6}
    Self-attention(\mathbf{Q,K,V}) = softmax(\frac{\mathbf{QK}^T}{\sqrt{d_k}}) \mathbf{V}
\end{equation}, where $\mathbf{Q}$, $\mathbf{K}$, and $\mathbf{V}$ are the Query weighted matrix, Key weighted matrix and Value weighted matrix, respectively. $d_k$ is the dimension of the $\mathbf{K}$ or $\mathbf{Q}$.}}



%-mentioned attention computations are repeated multiple times in parallel, each with a different set of learned weights for $\mathbf{W_Q},\mathbf{W_K},$ and $\mathbf{W_V}$.}\DEL{Each of \tannsdi{these computation processes} (??what is "these"?-done) is called an \emph{Attention Head~\cite{attention-head}. The calculated attention  or weights are maintained in a KV-cache.}}

The FC2 layer outputs logits, which is passed through the Add to generate the probabilities of words in the vocabulary. %and then the next new token.
The above operations are executed by each attention head in parallel. %Each attention head uses its own set of Query, Key, and Value parameters.
%This allows the model to capture various aspects of the context and focus on different relationships among words simultaneously~\cite{Vaswani2017AttentionIA}.
%The Attention module splits its Query, Key, and Value parameters N-ways and passes each split independently through a separate Head
Finally, the results from all attention heads are concatenated. %The concatenated results form a new matrix for each word in the sentence.
%This new matrix is later used to produce the final attention score. 
